Detection and Evaluation of human and machine generated speech in spoofing attacks on automatic speaker verification systems

Automatic speaker verification (ASV) systems utilize the biometric information in human speech to verify the speaker's identity. The techniques used for performing speaker verification are often vulnerable to malicious attacks that attempt to induce the ASV system to return wrong results, allowing an impostor to bypass the system and gain access. Attackers use a multitude of spoofing techniques for this, such as voice conversion, audio replay, speech synthesis, etc. In recent years, easily available tools to generate deepfaked audio have increased the potential threat to ASV systems. In this paper, we compare the potential of human impersonation (voice disguise) based attacks with attacks based on machine-generated speech, on black-box and white-box ASV systems. We also study countermeasures by using features that capture the unique aspects of human speech production, under the hypothesis that machines cannot emulate many of the fine-level intricacies of the human speech production mechanism. We show that fundamental frequency sequence-related entropy, spectral envelope, and aperiodic parameters are promising candidates for robust detection of deepfaked speech generated by unknown methods.

==> generatePairs.tex <==
ASVspoof2019 dataset contains logical access data and physical access data. In this study, we only use the logical access data which contains machine-generated speech using multiple text-to-speech synthesis and voice conversion methods. The logical data has 2580 bonafide utterances and 22800 synthetic utterances from 20 speakers in the training set; 2548 bonafide utterances from 20 speakers and 22296 spoof utterances from 10 speakers in the development set \cite{todisco2019asvspoof}. The evaluation set contains 7355 bonafide utterances from 67 speakers and 63882 spoof utterances from 48 speakers. The spoof audios are generated using unseen spoofing algorithms intentionally, aiming to give insights of the generalization performance of the proposed countermeasure models. In order for a general ASV system to evaluate this dataset, we generate 4914 positive pairs and 4914 negative pairs for each attack(A07-A19) from original evaluation set. We also generate 15970 positive pairs and 15970 negative pairs to evaluate the overall attacking ability over all attacks. 



 \textit{ASVspoof Evaluation Pairs:} Original ASVSpoof2019 dataset only contains stand-alone samples, however, typical ASV evaluates pairs. Methods of generating pairs vary and following is one possible of them. In ASVSpoof2019 logical access(LA) evaluation set, each type of attack generates 4914 spoof utterances. Selection of negative pairs follows the algorithm \ref{negativepairs}, which should give 13 pieces of 4914 negative pairs. Selection of positive pairs is more trivial by following the criterion that the number of any speaker in the resulting pairs is approximately proportional to the number of that speaker in all bonafide utterances in the original evaluation set. We balance negative and positive pairs as VoxCeleb1 test set does, which is to say, there are 4914 positive pairs given an attack and this will give 13 pieces of 9828 pairs corresponding to 13 attacks(A07-A19). To evaluate the overall performance of spoof attack, we also build balanced "all-embracing" pairs through the following way: combine all 13 pieces of negative pairs and randomly select one quarter of them as "all-embracing negative pairs"; generate positive pairs using the same method as mentioned above. This will finally give 31940 pairs. We note this as \textit{A-ALL}. Both our Black Box and White Box will evaluate on these data sets.

\textit{ASVspoof Training Identities:} To furthermore fine tune Black Boxes or train White Boxes, the initial ASVspoof2019 training set needs to be "expanded" based on the following assumption: if $(A_i, j)$ represents the $i_{th}$ attack to the $j_{th}$ speaker, then $(A_i, j)$ could be defined as a unique "speaker". For the ASVspoof2019 training set, there are 20 speakers and 6 types of attack. Thus there will be 120 spoof "speakers". Applying the strategy above, new training set will contain 25380 utterances from 140 speakers.  

\begin{algorithm}
\caption{\textbf{Generating Negative Pairs} } 
\begin{algorithmic}[1]
\For{$k=1,...,\#$ of speakers}
\State {$dict[k] \leftarrow hashset\{\}$}
\EndFor
\For{$x=1,...,\#$ of bonafide samples}
\State Get identity as $id_x$
\State {Add x into $dict[id_x]$}
\EndFor
\For{attack in A07-A19}
\State{make a copy $dict_c \leftarrow dict$}
\For{utterance $x_1$ in all of 4914 samples}
\State{Get identity as $id_{x_1}$}
\State{Randomly select a sample $x_2$ from $dict_c[id_{x_1}]$ and remove $x_2$ from $dict_c[id_{x_1}]$}
\State{Save pair$(x_1, x_2)$ for current attack}
\EndFor
\EndFor
\end{algorithmic}
\label{negativepairs}
\end{algorithm}
